Egocentric Audio-Visual Noise Suppression

This paper studies audio-visual noise suppression for egocentric videos -- where the speaker is not captured in the video. Instead, potential noise sources are visible on screen with the camera emulating the off-screen speaker's view of the outside world. This setting is different from prior work in audio-visual speech enhancement that relies on lip and facial visuals. In this paper, we first demonstrate that egocentric visual information is helpful for noise suppression. We compare object recognition and action classification-based visual feature extractors and investigate methods to align audio and visual representations. Then, we examine different fusion strategies for the aligned features, and locations within the noise suppression model to incorporate visual information. Experiments demonstrate that visual features are most helpful when used to generate additive correction masks. Finally, in order to ensure that the visual features are discriminative with respect to different noise types, we introduce a multi-task learning framework that jointly optimizes audio-visual noise suppression and video-based acoustic event detection. This proposed multi-task framework outperforms the audio-only baseline on all metrics, including a 0.16 PESQ improvement. Extensive ablations reveal the improved performance of the proposed model with multiple active distractors, overall noise types, and across different SNRs.

==> sections/background.tex <==


% \subsection{Related Work}

% Noise suppression has evolved over the years, from methods like Spectral Subtraction to now neural network approaches for enhancement in the time and frequency domains. 

% \textbf{ROSHAN: TODO }



% \subsection{}
% Explain Noise Suppression using the FERRARIS framework here








==> sections/setup.tex <==
\subsection{Dataset and Input Features}

Audioset~\cite{Audioset} is a large scale dataset of videos extracted from the wild which is used as the noise source. These 10-second videos describe different acoustic events in diverse visual environments. Off-screen target speech is derived from the Deep Noise Suppression (DNS) Challenge~\cite{reddy2021interspeech}. The distractor audio and target clean off-screen speech are combined after volume normalization by sampling a mixing SNR $s \sim N(0,5)$. The video is resampled to 2 fps.
%and resizing the video to have minimum dimension of 224 to be compatible with object detection feature extractors. 

Test sets are created for evaluation using the same mechanism as the training data preparation with the test sets of Audioset.  We select a small subset of 20 samples of this data for AB format human evaluation between the baseline and our approach.


% In order to perform evaluation using ASR, we create an ASR test set by mixing audio set evaluation data with Librispeech test-clean utterances. We randomly sample a test-clean utterance for every distractor video in the Audioset. 


%The audio-visual data that represents distractor sources is derived from the public Audioset dataset.







% The baseline model has a convolutional down-sampling encoder with 5 layers, each with kernel size $(2,4)$. The stride is $(1,2)$, with the layers having 16, 32, 64, 76, and 98 convolutional channels. The recurrent processor is composed of 4 latency-controlled bidirectional LSTM layers with a context of 60 frames. The models are trained using a STFT weighted L1 perceptual loss, a logSISDR loss and an unweighted L1 loss on the STFT output. The loss weights are 22.62, 0.001 and 1.0 respectively. An Adam optimizer is employed for optimization with a peak learning rate of 0.009 and a batch size of 84 across 32 GPUs.   

\subsection{Evaluation Metrics}

Noise Suppression models are evaluated using both objective and subjective speech quality metrics. For objective evaluation, we use PESQ \cite{PESQ}, STOI \cite{STOI}, and VISQOL \cite{VISQOL}. We also obtain DNSMOS and AB format human evaluation for our models. 

% \par In addition we assess the quality of proposed methods for speech enhancement by decoding the enhanced speech with an \gls{ASR} model. We train a multi-style \gls{ASR} model on the LibriSpeech dataset \cite{panayotov2015librispeech}, which contains 960 hours of clean English read speech. Specifically, with a probability of 50\%, we randomly mix a clean speech sample from LibriSpeech and a distractor sample from AudioSet training split with 5dB \gls{SNR}. Our \gls{ASR} is a streaming RNN-T model, which consists of 20 Emformer \cite{shi2021emformer} encoder layers, three LSTM \cite{hochreiter1997long} predictor layers, and a joiner layer with a vocabulary of 4,096 word piece units. We train the \gls{ASR} model for 150 epochs with the peak learning rate of $1e-4$  with 10k warm-up steps and an exponential decay with a factor 0.96 after 60 epochs. 
